Measuring Urban Deprivation from User Generated Content

Measuring socioeconomic deprivation of cities in an accurate and timely fashion has become a priority for governments around the world, as the massive urbanization process we are witnessing is causing high levels of inequalities which require intervention. Traditionally, deprivation indexes have been derived from census data, which is however very expensive to obtain, and thus acquired only every few years. Alternative computational methods have been proposed in recent years to automatically extract proxies of deprivation at a fine spatio-temporal level of granularity; however, they usually require access to datasets (e.g., call details records) that are not publicly available to governments and agencies. To remedy this, we propose a new method to automatically mine deprivation at a fine level of spatio-temporal granularity that only requires access to freely available user-generated content. More precisely, the method needs access to datasets describing what urban elements are present in the physical environment; examples of such datasets are Foursquare and OpenStreetMap. Using these datasets, we quantitatively describe neighborhoods by means of a metric, called {\em Offering Advantage}, that reflects which urban elements are distinctive features of each neighborhood. We then use that metric to {\em (i)} build accurate classifiers of urban deprivation and {\em (ii)} interpret the outcomes through thematic analysis. We apply the method to three UK urban areas of different scale and elaborate on the results in terms of precision and recall.

==> conclusions.tex <==
World is undergoing a process of fast urbanization. Urban poverty and inequality seem on the rise since some areas benefit more than others of public investments and economic growth. To counteract this issue, aid agencies are searching for novel ways to quantify and localize deprivation. Actual methods to achieve this are based on the analysis of survey data which, although accurate and reliable, is expansive, not kept updated and difficult to understand for non-experts. In this work, we present a method to map deprivation which tries to overcome these limitations. To this end, we extract physical features of the urban environment from two user generated content datasets -- Foursquare and OSM -- for 3 UK cities and we study the relationships between those features and the UK Indexes of Multiple Deprivation. We find strong associations between some urban features and deprivation scores. Moreover, we build a conceptual categorization for those features which are common across the case studies and which have the same relationships with deprivation. This approach provides three main advantages on actual methods. Firstly, data used for the analysis is free of charge and easily accessible. Secondly, since data for the analysis is constantly kept updated by users and developers, our method provides outcomes in real time. Finally, the thematic categorization proposed improves readability of results so that a wide public can understand, share and use them.

We account for four limitations. While IMD dataset contains information dating back to 2011, Foursquare and OSM datasets contain updated information. This time discrepancy might lead to inaccurate results since it is not demonstrated that relationships between urban features and deprivation are stable over time. Both Foursquare and OSM datasets have geographical and social biases. The two datasets, in fact, do not have a uniform coverage across space and most of the data tend to be concentrated in cities' cores. The social bias is related to the fact that both Foursquare and OSM users are not a representative group for the entire population thus geographical contributions might be biased by their specific interests or aims. The final limitation relates to dataset structures. Foursquare and OSM datasets have categories not fully structured and POIs which are supposed to belong to the same category and assigned to different categories at times.

We suggest two future developments for this work. We demonstrate that it is possible to extract urban features from two user generated content datasets to find insights about deprivation. We hypothesize that outcomes of this work can be improved by integrating in the analysis other urban features (e.g. street segments) which might be extracted from the same or from other user generated content datasets. We also suggest that, after having carried out the necessary improvements, our method can be useful for quantifying and localizing deprivation in developing countries which more than others need this assessment.    






%\begin{itemize}
%  \item {General wrap up.}
%  \item {Limitations.}
  
%    \begin{itemize}
%    \item Time discrepancies between datasets.
%    \item Geographical bias.
%    \item Social bias. 
%   \item Foursquare and OSM are not fully structured (fragmented).
%    \end{itemize}   
  
%  \item {Future work.}

%    \begin{itemize}
%    \item Foursquare + OSM + street network to improve knowledge about cities. 
%    \item Extend this work to developing countries which need, more than others, poverty indexes.
%    \end{itemize} 

%\end{itemize} 
